ROOAD: RELLIS Off-road Odometry Analysis Dataset

The development and implementation of visual-inertial odometry (VIO) has focused on structured environments, but interest in localization in off-road environments is growing. In this paper, we present the RELLIS Off-road Odometry Analysis Dataset (ROOAD) which provides high-quality, time-synchronized off-road monocular visual-inertial data sequences to further the development of related research. We evaluated the dataset on two state-of-the-art VIO algorithms, (1) Open-VINS and (2) VINS-Fusion. Our findings indicate that both algorithms perform 2 to 30 times worse on the ROOAD dataset compared to their performance in structured environments. Furthermore, OpenVINS has better tracking stability and real-time performance than VINS-Fusion in the off-road environment, while VINS-Fusion outperformed OpenVINS in tracking accuracy in several data sequences. Since the camera-IMU calibration tool from Kalibr toolkit is used extensively in this work, we have included several calibration data sequences. Our hand measurements show Kalibr's tool achieved +/-1 degree for orientation error and +/-1 mm at best (x- and y-axis) and +/-10 mm (z-axis) at worse for position error in the camera frame between the camera and IMU. This novel dataset provides a new set of scenarios for researchers to design and test their localization algorithms on, as well as critical insights in the current performance of VIO in off-road environments. ROOAD Dataset: github.com/unmannedlab/ROOAD

==> figures/datasetperf.tex <==
\begin{table*}[h]
\centering
\vspace{10pt}
\captionsetup{margin={0pt,0pt}}
\caption{Absolute Trajectory Error Performance of OpenVINS}
\begin{tabular}{c|c|c|c|c}
\hline
File Name             & RMSE Orientation       & STD Orientation & RMSE Position & STD Position  \\
\hline
rt4\_gravel            & 177.1        & 1.7       & 1.4     & 0.7 \\
\hline
rt4\_rim               & 175.9        & 2.7       & 1.2      & 0.3 \\
\hline
rt4\_updown            & 175.9        & 2.4       & 5.0     & 2.0 \\
\hline
rt5\_gravel            & 177.33        & 1.718       & 0.747      & 0.235  \\
\hline
rt5\_rim               & 175.664       & 2.992        & 1.23       & 0.526  \\
\hline
rt5\_updown            & 175.755       & 2.313        & 1.191    & 0.366  \\
\hline
\end{tabular}

\begin{tablenotes}
    \centering
    \small
    \item TODO: Find what to use for standard deviation

\end{tablenotes}

\label{tbl:datasetate}
\vspace{-10pt}

\end{table*}


==> figures/datasetrelperf.tex <==
\begin{table*}[h]
\centering
\vspace{10pt}
\captionsetup{margin={0pt,0pt}}
\caption{Relative pose error of OpenVINS for the provided datasets.}
\begin{tabular}{c|c|c|c|c|c}
\hline
File Name              & 8m             & 16m         & 24m          & 32m           & 40m         \\
\hline
rt4\_gravel            & 4.859\textdegree /10.243m   & 6.509\textdegree /20.574m & 8.529\textdegree /30.798m & 19.499\textdegree /38.988m & 45.240\textdegree /45.088m \\
\hline
rt4\_rim               & 50.018/12.054 & 93.320/18.903 & 155.675/18.779 & 157.839/20.591 & 129.101/21.322 \\
\hline
rt4\_updown            & 11.143/11.566 & 16.984/22.015 & 22.429/31.885  & 29.350/39.730  & 36.618/49.192 \\
\hline
rt5\_gravel            & 4.495/10.023  & 7.153/18.589  & 12.783/26.799  & 31.753/33.436  & 75.229/40.043 \\
\hline
rt5\_rim               & 51.058/12.086 & 102.946/18.63 & 166.22/17.039  & 140.9/15.546   & 106.619/17.259  \\
\hline
rt5\_updown            & 9.21/11.942   & 19.394/19.446 & 30.026/23.141  & 39.856/27.163 & 56.489/29.695  \\
\hline
\end{tabular}

\begin{tablenotes}
    \centering
    \small
    \item TODO: Establish Units and make table more readable
\end{tablenotes}
\label{tbl:datasetrpe}
\vspace{-10pt}

\end{table*}


==> figures/panorama.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{images/panarama.png}
  \caption{Panorama image of the testing location's sinkhole. [TODO: Replace with a Panorama @ Noon on the eroded plateau.]}
  \label{fig:panorama}
\end{figure*}

==> figures/rt4_gravel_path_err.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{images/rt4_gravel_err.pdf}
  \caption{Evening gravel path trajectory error with respect to the ground truth GPS coordinates. Evaluation performed using the RPG Trajectory Tool box\cite{Zhang18iros}. (Units: mm) }
  \label{fig:rt4gravelerr}
\end{figure}
\vspace{-5pt}

==> figures/rt4_gravel_path_xy.tex <==
\begin{figure}
  \centering
  \includegraphics[width=0.5\textwidth]{images/rt4_gravel_top_traj.pdf}
  \caption{Evening gravel path trajectory predicted by the VIO algorithm compared to the RTK GPS ground truth data. Evaluation performed using the RPG Trajectory Tool box\cite{Zhang18iros}. (Units: m) }
  \label{fig:rt4gravelxy}
\end{figure}
\vspace{-5pt}

==> figures/trajectory_estimate_topdown_gravel.tex <==

\begin{figure*}[h]
\centering
\vspace{10pt}
\captionsetup{margin={0pt,0pt}}

\begin{tabular}{cc}

 (1) OpenVINS             & (2) VINS-Fusion \\

 %\begin{tabular}{l} 
 %(a) 
 %\end{tabular} &  
 %\includegraphics[width=0.45\textwidth]{images/OV_traj/rt4_gravel/trajectory_top_posyaw_-1.pdf} &
 %\includegraphics[width=0.45\textwidth]{images/VF_traj/rt4_gravel/trajectory_top_posyaw_-1.pdf} \\

 %\begin{tabular}{l} 
 %(b)  
 %\end{tabular} & 
 %\includegraphics[width=0.45\textwidth]{images/OV_traj/rt4_rim/trajectory_top_posyaw_-1.pdf} &
 %\includegraphics[width=0.45\textwidth]{images/VF_traj/rt4_rim/trajectory_top_posyaw_-1.pdf} \\

 %\begin{tabular}{l} 
 %(c) 
 %\end{tabular} & 
 \includegraphics[width=0.45\textwidth]{images/OV_traj/rt4_gravel/trajectory_top_posyaw_-1.pdf} &
 \includegraphics[width=0.45\textwidth]{images/VF_traj/rt4_gravel/trajectory_top_posyaw_-1.pdf} \\

\end{tabular}

%\begin{tablenotes}
%    \centering
%    \small
%\end{tablenotes}

\vspace{-10pt}
%\caption{Comparison of trajectory estimates aligned to ground truth GPS. (a) represents the gravel path, (b) represents the rim path, and (c) represents the up-down path. (Units: m)}
\caption{Comparison of trajectory estimates aligned to ground truth GPS of the Gravel path (Units: m)}
\label{fig:trajectoryerrortopdown}
\end{figure*}


==> figures/trajectory_estimate_topdown_rim.tex <==

\begin{figure*}[h]
\centering
\vspace{10pt}
\captionsetup{margin={0pt,0pt}}

\begin{tabular}{cc}

 (1) OpenVINS             & (2) VINS-Fusion \\

 %\begin{tabular}{l} 
 %(a) 
 %\end{tabular} &  
 %\includegraphics[width=0.45\textwidth]{images/OV_traj/rt4_gravel/trajectory_top_posyaw_-1.pdf} &
 %\includegraphics[width=0.45\textwidth]{images/VF_traj/rt4_gravel/trajectory_top_posyaw_-1.pdf} \\

 %\begin{tabular}{l} 
 %(b)  
 %\end{tabular} & 
 %\includegraphics[width=0.45\textwidth]{images/OV_traj/rt4_rim/trajectory_top_posyaw_-1.pdf} &
 %\includegraphics[width=0.45\textwidth]{images/VF_traj/rt4_rim/trajectory_top_posyaw_-1.pdf} \\

 %\begin{tabular}{l} 
 %(c) 
 %\end{tabular} & 
 \includegraphics[width=0.45\textwidth]{images/OV_traj/rt4_rim/trajectory_top_posyaw_-1.pdf} &
 \includegraphics[width=0.45\textwidth]{images/VF_traj/rt4_rim/trajectory_top_posyaw_-1.pdf} \\

\end{tabular}

%\begin{tablenotes}
%    \centering
%    \small
%\end{tablenotes}

\vspace{-10pt}
%\caption{Comparison of trajectory estimates aligned to ground truth GPS. (a) represents the gravel path, (b) represents the rim path, and (c) represents the up-down path. (Units: m)}
\caption{Comparison of trajectory estimates aligned to ground truth GPS of the Rim path (Units: m)}
\label{fig:trajectoryerrortopdown}
\end{figure*}

